Reconciling Reality through Simulation: A Real-to-Sim-to-Real Approach for Robust Manipulation

Imitation learning methods need significant human supervision to learn policies robust to changes in object poses, physical disturbances, and visual distractors. Reinforcement learning, on the other hand, can explore the environment autonomously to learn robust behaviors but may require impractical amounts of unsafe real-world data collection. To learn performant, robust policies without the burden of unsafe real-world data collection or extensive human supervision, we propose RialTo, a system for robustifying real-world imitation learning policies via reinforcement learning in "digital twin" simulation environments constructed on the fly from small amounts of real-world data. To enable this real-to-sim-to-real pipeline, RialTo proposes an easy-to-use interface for quickly scanning and constructing digital twins of real-world environments. We also introduce a novel "inverse distillation" procedure for bringing real-world demonstrations into simulated environments for efficient fine-tuning, with minimal human intervention and engineering required. We evaluate RialTo across a variety of robotic manipulation problems in the real world, such as robustly stacking dishes on a rack, placing books on a shelf, and six other tasks. RialTo increases (over 67%) in policy robustness without requiring extensive human data collection. Project website and videos at https://real-to-sim-to-real.github.io/RialTo/

==> texs/rebuttal.tex <==
\onecolumn
\section{Rebuttal}

\subsection{General Response to Reviewers}
We thank all the reviewers for their useful feedback. % and for helping us make our submission stronger. 
%All the reviewers seem to agree about the novelty and interest of RialTo: \textit{"The paper introduces an innovative concept"} (JvjM), \textit{"The idea of using simulation replica to augment real data through RL is novel"} (7vyQ), \textit{"The idea of using real-to-sim-to-real is interesting and can reduce human effort during collecting demonstrations"} (uim6). There is agreement in the noteworthy of the system proposed: \textit{"the engineering of the system is robust"}(JvjM), \textit{"The aspect of creating a digital twin [...] is particularly noteworthy"}(JvjM), \textit{"the intuitive graphical interface can benefit other research in this community"} (uim6). The reviewers valued the experiments done to support our argument \textit{"The experiment is supportive of the claim"} (7vyQ), \textit{"The user study verifies the effectiveness of the GUI design"} (7vyQ). 
%
We address the reviewer's final questions and concerns with new material and corrections added in the paper in blue and in our response below. We also added several new videos in the supplementary material (inside the rebuttal\_videos folder named video\_X\_....mp4). We respond to each reviewer individually and we provide below a summary of the new material:
\begin{enumerate}
   \item \textit{[Reviewer JvjM]} Added 2 complex scenes and showed that RialTo can scale up to more complex scenes. (See Figure \ref{fig:inthewildenv} and video\_1)
    \item \textit{[Reviewer JvjM]} Proposed an approximate scaling law derived from our user study for the time needed for reconstructing complex 3D scenes with RialTo's GUI. We show the 3D reconstruction time scales linearly with the number of objects and joints in the scene (See Section \ref{apdx:scalinglawsscanning}). 
    \item \textit{[Reviewer JvjM]} We show how RialTo's GUI can successfully handle more complex scenes, like a kitchen with more articulations and objects (see video\_2) %, some articulated (See Video 2)
    \item \textit{[Reviewer uim6]} Trained a multi-task policy on four tasks. The performance of the multi-task policy matches the single-task policy performance but more data is needed to obtain positive transfer across tasks (See Section \ref{apdx:rialtomultitask}).
    \item Added further ablations comparing the use of real-world demos against simulated demos. We observe that real-world demos bring a significant improvement during co-training that is not obtained with simulated demos(See Fig. \ref{fig:cotrainingandrealvssim}).
   \item \textit{[Reviewer 7vyQ]} Provided further ablations on the quantity of real-world imitation data needed to bootstrap    RL-finetuning. We observe a step function relation, where we need enough real-world data for the real-world policy to transfer to simulation to do RL fine-tuning successfully (See Section \ref{apdx:rlrealworldablation}).
   \item \textit{[Reviewer 7vyQ]} Added an experiment training a policy on both synthetic assets and the target simulated environment on the opening drawer task. No improvement over training on the target environment was observed, we hypothesize that more data might be needed. (See Section \ref{apdx:mixsynthtarget})
   \item \textit{[Reviewer JvjM]} New imitation learning baseline with data augmentation adding scanned object meshes on the point cloud. No improvement was observed, the main benefit of RialTo comes from the RL fine-tuning in simulation which discovers recovery behaviors and robustness to object poses. These behaviors cannot be obtained without exploration or many more demonstrations. (See Section \ref{apdx:il++})
   \item \textit{[Reviewer uim6]} New videos for opening the cabinet with the cabinet fixed and a softer impedance controller. (video\_3)
   \item \textit{[Reviewer uim6]} Improved Figure 3 for more clarity. (See Figure \ref{fig:real2sim-policy})
   \item Added error bars in all plots and tables. (See Fig \ref{fig:mainres}, Table \ref{tab:extrail}, Fig \ref{fig:simbaseline}) 
   \item \textit{[Reviewer JvjM]} Expanded the conclusion and limitations sections. (See Section \ref{sec:conclusion})
\end{enumerate}


\subsection{Response to Reviewer JvjM}
Dear reviewer JvjM,

Thank you for reviewing our work and providing helpful feedback. Please find detailed responses to your comments below:
% Firstly, we want to thank you for your time reviewing our work and for providing feedback that will help us convey more clearly the strength of our work. Please find a detailed response to your comments below:

\textit{\textbf{It is not very clear how RialTo scales to more complex scenes.}}

%Your concerns about further understanding the scalability of RialTo's 3D reconstruction are valid. %well addressed.
% We do the following experiments to answer it:
We performed the following experiments to highlight further that RialTo is a scalable pipeline:
\begin{enumerate}
    \item We provide 2 new experiments of scaling RialTo to more ``in-the-wild" complex scenes. We show that RialTo learns a successful policy in these challenging scenes. The two tasks in different kitchen settings consist of putting a cup in the trash and a dish from the sink to the dish rack. (See Section \ref{sec:rialtowild} and video\_1)
    \item We show RialTo's reconstruction pipeline can handle a more complex kitchen scene containing an articulated oven and sandwich maker, and additional free (a lemon and a jar). It took 20 minutes for an expert user to reconstruct this scene (See video\_2)
    \item We provide an approximate scaling law with the numbers extracted from our user study showing the linear scaling properties of RialTo's reconstruction pipeline.
    \begin{equation}
    \label{eq:scalingrebut}
    \begin{split}
                total\_active\_time = (3:14) \\+ (4:50) \cdot N_{\textit{objects}}\\ + (3:40) \cdot N_{\textit{cut objects}}\\ + (2:54) \cdot N_{joints}
    \end{split}   
\end{equation}
This relation shows time increases linearly with the number of objects and articulations. However, this effort will be reduced once learning methods can extract articulations and meshes autonomously, for which RialTo's pipeline is compatible. (see Section \ref{apdx:scalinglawsscanning} for more details)
\end{enumerate}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/rialtointhewildv2.pdf}
    \caption{\footnotesize{We test \MethodName on uncontrolled and in-the-wild scenes, and we see we can continue to solve a variety of tasks more robustly than imitation learning techniques. (See original Figure in \ref{fig:inthewildenv})} }
    \label{reb:inthewildenv}
\end{figure}



\textit{\textbf{The paper provides insufficient detail regarding the real-to-sim reconstruction process. }}

We expand Section \ref{apdx:r2simscenes}, giving additional details on how each third-party software was used in combination with RialTo's GUI. Briefly, we use:
\begin{enumerate}
    \item \textbf{PolyCam} for extracting meshes of big scenes (e.g., the kitchens)
    \item \textbf{ARCode} for extracting meshes of single objects (e.g., mug, cabinet, drawer)
    \item \textbf{NeRFStudio} for extracting meshes of single objects with fine details (e.g., the dish rack)
    \item \textbf{RialTo's GUI} to specify separate bodies, joints, and the kinematics of the scene (the code for this GUI will be released with the rest of the code), see Figure \ref{fig:real2simpipeline-simgeneration}. 
\end{enumerate}. 
%
%This GUI offers a method for generating digital twin assets with a small amount of human effort, as fully automated tools for reconstructing textured scene geometry with full joints and articulated kinematics are still not readily available.
% This GUI makes the digital-twin generation possible as long as the technology for inferring joints and kinematics autonomously is not developed. 

\textit{\textbf{The paper omits discussion of other studies that have improved the robustness of learned imitation learning policies using 2D and generative models.}}
\begin{table}[h!]
\centering
\begin{tabularx}{0.5\linewidth}{@{}lc*{5}{>{\centering\arraybackslash}X}@{}}
\toprule
 & Pose & Distractors & Disturbances \\ %& Open \\
 & randomization &  &  \\ % &  cabinet  \\
\midrule
\addlinespace
IL & \textbf{40} $\pm$ 15\% & \textbf{50} $\pm$ 17\% & \textbf{10} $\pm$ 9\%\\ % & - \\
IL with distractors &  \textbf{50} $\pm$ 17\% & 20 $\pm$ 13\%  & \textbf{10} $\pm$ 9\% \\ % & - \\
\bottomrule
\end{tabularx}
\caption{Comparison of the plain imitation learning baseline (IL) against adding new distractors (IL with distractors) on the task of opening the drawer. No improvement is observed. (See original table \ref{tab:il++})}
\label{reb:il++}
\vspace{-15pt}
\end{table}


We now acknowledge this work in our related work section (See Section~\ref{sec:relatedwork}). Furthermore, we provide new experiments comparing \textbf{RialTo} to an equivalent baseline in the 3D space (see Section \ref{apdx:il++}).
\begin{itemize}
    \item \textit{Method}: We train imitation learning policies from real-world demonstrations adding scanned/generated 3D assets merged to the point cloud to make the policies more robust to visual distractors
    \item \textit{Results}: in Table \ref{tab:il++} we observe that this method did not increase the performance of the imitation learning baseline. 
    \item \textit{Conclusion}: We hypothesize that more intelligent augmentations need to be performed to simulate occlusions in the 3D point clouds. Nevertheless, even if these augmentation techniques could make the policy more robust to object distractors, they could not show the recovery behaviors and robustness to physical disturbances seen in RialTo which comes from the RL fine-tuning phase, if not demonstrated.
\end{itemize}

\textit{\textbf{What are types of robustness that cannot be achieved by this approach?}}

We expanded the limitations section to include this answer (See \ref{sec:conclusion}). In theory, this approach should extend to obtain robustness in all that can be simulated, e.g. lighting, object shapes, variations of clutter. However, it will not be able to be robust to things that cannot be simulated, e.g. liquids and deformables. Similarly, highly dynamic tasks will need a more extensive real-world identification. Nevertheless, a significant body of work is proposing new techniques for doing system identification and simulating deformables which shows the great potential of methods like RialTo that leverage the simulation. Finally, RialTo relies on a few demonstrations, thereafter it will fail with those tasks that cannot be demonstrated by a human.

\subsection{Response to Reviewer uim6}
Dear reviewer uim6,

Thank you for reviewing our work and providing helpful feedback. Please find detailed responses to your comments below:

\textit{\textbf{I strongly suggest the authors add an experiment to show the performance of the proposed approach when it’s trained on diverse datasets across different tasks.}}

\begin{table}[h!]
\centering
\begin{tabularx}{0.5\linewidth}{@{}lc*{5}{>{\centering\arraybackslash}X}@{}}
\toprule
 & Open & Mug  \\ %& Open \\
 & drawer& on shelf \\ % &  cabinet  \\
\midrule
\addlinespace
Imitation learning  & 40 $\pm$ 17\% & 10 $\pm$ 9\%\\ % & - \\
\MethodName & \textbf{90} $\pm$ 9\% & \textbf{100} $\pm$ 0\%\\ % & - \\
\MethodName multitask &  \textbf{90} $\pm$ 9\% & 80 $\pm$ 15\% \\ % & - \\
\bottomrule
\end{tabularx}
\caption{Comparison of training \MethodName on multiple tasks against single-task \MethodName. No improvement is observed.(See original table in \ref{tab:multitaskrialto})}
\label{reb:multitaskrialto}
\vspace{-15pt}
\end{table}

\textit{Method}: We trained a multi-task policy on 4 of the environments: opening a drawer, putting a mug on a shelf, throwing the cup in the trash, and putting a plate on the rack (see Section \ref{apdx:rialtomultitask}). The adapted \textit{multi-task} version of \textbf{RialTo} is the following:

\begin{enumerate}
    \item  Train separate state-based single-task policies per task
    \item  Collect trajectories from each one of the tasks with the state-based policies
    \item  Distill these trajectories into a single multi-task policy conditioned with the task-id
    \item Run multiple iterations of DAgger on each task sequentially to obtain a final multi-task policy
\end{enumerate}
%
\textit{Evaluation}: We evaluate this policy in the real world on two of the tasks and observe that in \emph{opening the drawer}, the performance of multi-task \textbf{RialTo} matches single-task (90\% success). However, the performance slightly decreases on the \emph{mug on the shelf task} (from 100\% on single-task to 80\% on multi-task). The performance is above the imitation learning baseline (40\% for the drawer and 10\% for the mug on the shelf).
We did not tune any hyperparameters, and we kept the same network size that we used for the \textbf{RialTo} experiments. We should be able to bring the performance of the mug on the shelf task to match the single-task policy with some hyperparameter tuning. 

\textit{Conclusion}: We showed that \textbf{RialTo} can be easily adapted to train multi-task policies. Nevertheless, we need to train in more environments to obtain multi-task generalization.


\textit{\textbf{Clarification on inputs of the policies in Fig. 3.}}

We improved Figure 3 by writing the name of the observation for each one of the policy inputs (see Figure \ref{fig:real2sim-policy}). To clarify further:
\begin{enumerate}
    \item The real-world imitation learned policy takes point clouds and end-effector poses as inputs.
    \item This policy is then inverse-distilled into a state-based policy taking object poses and end effector poses for more efficient RL fine-tuning in simulation.
    \item We do teacher-student distillation to transfer this policy to the real world taking point clouds and end-effector poses as input (this last step is the teacher-student distillation procedure as done in \cite{chen2023visual} and is not shown in Figure 3 since it is not part of the novel inverse-distillation procedure).
\end{enumerate}

\textit{\textbf{The demo with “Open Cabinet” will look more realistic with a fixed cabinet. Could this be improved by a descent impedance controller?}}

Please, see video\_3 in the supplementary material where we fix the cabinet and run a smoother impedance controller.


\subsection{Response to Reviewer 7vyq}
Dear reviewer 7vyq,

Thank you for reviewing our work and providing helpful feedback. Please find detailed responses to your comments below:

\textit{\textbf{How sensitive is the algorithm to the quality/quantity of the initial real-world demonstration?}}

\begin{table}[h!]
\centering
\begin{tabularx}{0.5\linewidth}{@{}lc*{5}{>{\centering\arraybackslash}X}@{}}
\toprule
 & Book on & Open \\ %& Open \\
 & shelf & drawer  \\ % &  cabinet  \\
\midrule
\addlinespace
RL fine-tuning from 0 real demos & 0 $\pm$ 0\% & 0 $\pm$ 0\% \\ % & - \\
RL fine-tuning from 5 real demos &  0 $\pm$ 0\% & 89 $\pm$ 1\% \\ % & - \\
RL fine-tuning from 10 real demos &  0 $\pm$ 0\% & \textbf{96} $\pm$ 1\% \\ % & - \\
RL fine-tuning from 15 real demos &  \textbf{90} $\pm$ 1\% & \textbf{96} $\pm$ 1\% \\ % & - \\
\bottomrule
\end{tabularx}
\caption{Comparison of training RL from different amounts of real-world demos. (See original table in \ref{tab:realworlddemosablation})}
\label{reb:realworlddemosablation}
\vspace{-15pt}
\end{table}

\textit{Experiment}: We provide a new experiment showing the performance when varying the number of real-world demonstrations on the RL fine-tuning phase (See Section \ref{apdx:rlrealworldablation}). We start with 0,5,10, and 15 real-world demonstrations on the tasks of opening a drawer and putting a mug on a shelf. 

\textit{Results}: We observe a step-like performance variation with the number of demonstrations needed. This is because we need enough demonstrations for the real-world policy to transfer to the simulation in order to provide some successful trajectories. Otherwise, RL fine-tuning fails from sparse rewards with no simulated demonstrations. We observe that the task of opening a drawer needs 5 real-world demos to obtain an 89 \% success rate and 10 to obtain a 96\% success. On the other hand, putting a book on the shelf requires 15 real-world demos to obtain an 90\% success rate. With fewer demos, the real-world policy doesn't transfer to the simulation and obtains 0\% success.

\textit{\textbf{How is the reward designed during RL? if it's an imitation learning objective how does it handle large variations such as different object/robot positions?}}

The reward design for the RL fine-tuning is simple. \begin{itemize}
    \item We simply define a success metric (see Section \ref{appdx:taskdetails} for the exact metrics per task) and this is used as a sparse reward for the RL training
    \item We add an imitation learning objective as seen in Eq \ref{rl_finetune} (Note that this is not part of the reward function) to bias exploration and guide the policy towards real-world transferable policies.
\end{itemize}
The simple sparse reward and the IL objective together with the large GPU environment parallelization (2048 parallel environments) we are capable of finding solutions for object and robot position variations large enough to cover most of the robot's workspace without any dense reward or reward shaping (see Figure \ref{fig:taskoverview} for a depiction of the randomization done per task).

\textit{\textbf{Would combining the user-created scene with the synthetic scenes provide a further performance boost? that seems like a potential route to scale the algorithm up}}

\begin{table}[h!]
\centering
\begin{tabularx}{0.5\linewidth}{@{}lc*{5}{>{\centering\arraybackslash}X}@{}}
\toprule
 & Pose & Distractors  \\ %& Open \\
 & randomization & \\ % &  cabinet  \\
\midrule
\addlinespace
\MethodName & \textbf{90} $\pm$ 9\% & \textbf{90} $\pm$ 9\%\\ % & - \\
\MethodName + synthetic assets &  \textbf{90} $\pm$ 9\% & \textbf{80} $\pm$ 13\% \\ % & - \\
\bottomrule
\end{tabularx}
\caption{Comparison of using \MethodName with added synthetic assets against standard \MethodName on the task of opening the drawer in the real world. No improvement is observed. (see original figure in \ref{reb:combinesynthetictarget})}
\label{reb:combinesynthetictarget}
\vspace{-15pt}
\end{table}

\textit{Method}: We added a new experiment combining the user-created scene with synthetic ones for the tasks of opening the drawer to test this hypothesis. 

\textit{Results}: We provide the results in Section \ref{apdx:mixsynthtarget}. We see that no increase in performance is obtained compared to the standard imitation learning baseline. 

\textit{Conclusion}: More synthetic data might be needed to obtain an improvement. However, one of our claims is that collecting this synthetic dataset is challenging and time-consuming. It is tractable to collect this data for simple tasks like opening the drawer (for which the Objaverse dataset has data) however, this becomes a challenge for more visually complex tasks like putting a cup in a trash (see Fig \ref{fig:inthewildenv}). A promising avenue for scaling up \textbf{RialTo} would be to leverage RialTo's GUI and combine it with 3D generative and vision models to make digital twin generation more seamless and accurate. This would offer a potential pipeline for collecting a dataset large enough to start obtaining generalization and positive transfer across scenes.


\twocolumn
\setcounter{section}{0}
\setcounter{figure}{0}
